Measurement of the CPV Higgs mixing angle in ZZ-fusion at 1 TeV ILC

Although the studies of tensor structure of the Higgs boson interactions with vector bosons and fermions at CMS and ATLAS experiments have established that the $J^{\mathrm{PC}}$ quantum numbers of the Higgs boson should be $0^{++}$, small CP violation in the Higgs sector (up to 10% contribution of the CP-odd state) cannot be excluded with the current experimental precision. We review possibilities to measure CP violating mixing angle $\Psi_{\mathrm{CP}}$ between scalar and pseudoscalar states, at a linear electron-positron collider, at center-of-mass energy of 1 TeV.

==> concl.tex <==
\section{Conclusion}
\label{sec:concl}


==> ild.tex <==
\section{The ILD Concept and MC Samples}
\label{sec:ILDMC}
ILD~\cite{ILDIDR, ILDESU, TDR4} is one of the proposed detector concepts for future $e^+e^-$ Higgs factories.
It is highly-hermetic multi-purpose detector designed for particle flow reconstruction.
ILD consists of a high precision vertex detector, a time projection chamber, silicon tracking detectors, a highly granular calorimeter system and a forward detector system, all placed inside of a solenoid providing a magnetic field of $3.5$\,T, surrounded by an iron yoke instrumented for muon detection.
The jet energy resolution as a function of $|\cos \theta _{\mathrm{thrust}}|$ is shown in Fig.~\ref{fig:JER}.
Details of the ILD design, as well as about the particle flow concept can be found in Refs.~\cite{TDR4, LongESU, PFA}.

\begin{figure}[t]
\centering
\includegraphics[width = 8.4truecm]{./figures/JER_vs_cosTheta}
\caption{ILD jet energy resolution as function of $|\cos{\theta_{\mathrm{thrust}}}|$ for various fixed jet energies. From~\cite{ILDIDR}.}
\label{fig:JER}
\end{figure}


==> intro.tex <==
\section{Introduction}
\label{sec:intro}



\begin{table}[t]
\centering
\caption{}
\begin{tabular}{cccccc}
\hline
& &  &  &   &  \\
\hline
\end{tabular}
\label{tab:lumi}
\end{table}


==> recosel.tex <==
\section{High-level Reconstruction and Event Selection}
\label{sec:recosel}


==> results.tex <==
\section{Results}
\label{sec:results}

